A Survey on Industrial Internet of Things (IIoT) Testbeds for Connectivity Research

Industrial Internet of Things (IIoT) technologies have revolutionized industrial processes, enabling smart automation, real-time data analytics, and improved operational efficiency across diverse industry sectors. IIoT testbeds play a critical role in advancing IIoT research and development (R&D) to provide controlled environments for technology evaluation before their real-world deployment. In this article, we conduct a comprehensive literature review on existing IIoT testbeds, aiming to identify benchmark performance, research gaps and explore emerging trends in IIoT systems. We first review the state-of-the-art resource management solutions proposed for IIoT applications. We then categorize the reviewed testbeds according to their deployed communication protocols (including TSN, IEEE 802.15.4, IEEE 802.11 and 5G) and discuss the design and usage of each testbed. Driven by the knowledge gained during this study, we present suggestions and good practices for researchers and practitioners who are planning to design and develop IIoT testbeds for connectivity research.

==> Tables/tsn/others.tex <==
\begin{table*}[h]
\caption{Summary of Wired Testbeds based on Lagacy networks. }
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Type} & \textbf{Name (Authors.)} & \textbf{Inst.}                                                        & \textbf{Region}                                            & \textbf{Scenario} & \textbf{Func.}                                                     & \textbf{\begin{tabular}[c]{@{}l@{}}Num.\\ ES\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Num.\\ Bridge\end{tabular}} \\ \hline
PROFINET      & IORT  (Flammini et al.)        & \begin{tabular}[c]{@{}l@{}}University\\ of Brescia\end{tabular}       & \begin{tabular}[c]{@{}l@{}}Europe\\ (Italy)\end{tabular}   & General           & Low-delay                                                          & 115                                                        & 11                                                             \\ \hline
EtherCat      & Fastcat  (Brinkman et al.)     & Caltech                                                               & NA                                                         & Aerospace         & \begin{tabular}[c]{@{}l@{}}Low-delay, \\ Faulty\end{tabular}       & -                                                          & -                                                              \\ \hline
EtherCat      & (Delgado et al.)   & SeoulTech                                                             & Korea                                                      & Microgrid         & \begin{tabular}[c]{@{}l@{}}Low-delay, \\ Sync\end{tabular}         & 6                                                          & -                                                              \\ \hline
EtherCat      & (Lee et al.)       & \begin{tabular}[c]{@{}l@{}}Pusan\\ National\\ University\end{tabular} & Korea                                                      & Industrial        & \begin{tabular}[c]{@{}l@{}}Low-delay, \\ Sync\end{tabular}         & 6                                                          & -                                                              \\ \hline
EtherCat      & (Edelberg et al.)  & \begin{tabular}[c]{@{}l@{}}Caltech, \\ NASA\end{tabular}              & NA                                                         & Aerospace         & \begin{tabular}[c]{@{}l@{}}Low-delay, \\ Fault handle\end{tabular} & -                                                          & -                                                              \\ \hline
TTEthernet    & (Loveless et al.)  & NASA                                                                  & NA                                                         & Aerospace         & \begin{tabular}[c]{@{}l@{}}TT flow, \\ Sync\end{tabular}           & 7                                                          & 4                                                              \\ \hline
TTEthernet    & (Eramo et al.)     & \begin{tabular}[c]{@{}l@{}}University\\ of Rome\end{tabular}          & \begin{tabular}[c]{@{}l@{}}Europe\\ (Italy)\end{tabular}   & General           & \begin{tabular}[c]{@{}l@{}}TT flow, \\ Sync\end{tabular}           & 3                                                          & 1                                                              \\ \hline
TTEthernet    & (Craciunas et al.) & TTTech                                                                & \begin{tabular}[c]{@{}l@{}}Europe\\ (Austria)\end{tabular} & General           & \begin{tabular}[c]{@{}l@{}}TT flow, \\ Sync\end{tabular}           & 3                                                          & 1                                                              \\ \hline
TTEthernet    & (Yu et al.)        & \begin{tabular}[c]{@{}l@{}}Tsinghua\\ University\end{tabular}         & China                                                      & General           & \begin{tabular}[c]{@{}l@{}}Shaping, \\ Sync\end{tabular}           & 3                                                          & 2                                                              \\ \hline
\end{tabular}
}
\end{table*}

==> Tables/tsn/sim.tex <==
\begin{table}[]
\caption{Summary of Simulated TSN Testbeds. }
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\textbf{ID}} & \multicolumn{1}{c|}{\textbf{Authors}} & \multicolumn{1}{c|}{\textbf{Inst.}}                                  & \multicolumn{1}{c|}{\textbf{Scenario}} & \multicolumn{1}{c|}{\textbf{Support Func.}}                   & \multicolumn{1}{c|}{\textbf{Impl.}} \\ \hline
Dual                              & Jiang et al.                          & \begin{tabular}[c]{@{}l@{}}Hanyang\\ University\end{tabular}         & General                                & IEEE 802.1Qbv                                                 & OMNET++                             \\ \hline
OPNET                             & Pahlevan et al.                       & \begin{tabular}[c]{@{}l@{}}University\\ of Siegen\end{tabular}       & Sync                        & IEEE 802.1AS                                                  & OPNET                               \\ \hline
NS3                               & \begin{tabular}[c]{@{}l@{}}Krummacker \\et al.\end{tabular}                     & DFKI                                                                 & General                                & IEEE 802.1Qbv                                                 & NS-3                                 \\ \hline
TSimNet                           & Heise et al.                          & \begin{tabular}[c]{@{}l@{}}Airbus\\ Group\\ Innovations\end{tabular} & General                                & \begin{tabular}[c]{@{}l@{}}IEEE 802.1Qci, \\ Qbu\end{tabular} & OMNeT++                             \\ \hline
\end{tabular}
}
\end{table}

==> sec/notes.tex <==
\section{Layout of Survey}
Internet of Things (IoT), inter-networking of physical devices with computing and network connectivity, has also been referred to as ``the infrastructure of the information society". Not surprisingly, there has also been extensions of IoT to many other industry sectors such as medical (e.g., medical IoT), battlefields and military (e.g., battlefield / military IoT) and industrial (e.g., industrial IoT -- IIoT). IIoT, the focus of this paper, is the application of IoT technologies in industrial environments, including advanced manufacturing systems. Compared with IoT systems designed for consumer applications, IIoT systems designed for advanced manufacturing systems are usually deployed in harsh and complex environments, and have stringent dependability, timing performance (e.g., latency and jitter), energy-efficiency and security requirements to optimize manufacturing quality and productivity, and to avoid potentially catastrophic consequences. A more recent trend in advanced manufacturing is to connect interdependent factories together through IIoT technologies to provide decentralized, collaborative and sometimes immutable and verifiable services (e.g., distributed supply chain management). These unique requirements on IIoT systems pose many challenges in their communication fabric design, distributed data management, analysis and decision making, and security protection for both the communication and data infrastructure.

However, a scan of the existing literature (see Section ??? {\color{red}Raymond: to be updated after we have complete this paper}) highlights the lack of a representative testbed, in terms of size / scale, device diversity, etc. For example, most existing research efforts are limited at component level (sensing/control devices, controllers, etc.) or subsystem level (wireless edge networks, software-defined network (SDN) backbone, etc.), with performance evaluation/validation through simulation or small-scale experiments. This reinforces the importance of designing a scalable and flexible IIoT testbed that can serve as the networking and computing infrastructure to interconnect the components and subsystems. Such a testbed will benefit the research community by revealing the challenges underpinning complex and coupled systems, facilitating integrative studies on the system-level design, and allowing performance evaluation in large-scale realistic systems. In other words, having a scalable and flexible IIoT testbed will significantly boost existing research efforts, enhance the synergy of the various research projects, and enable future research that develops a holistic approach for IIoT systems.

Hence, in this paper we seek to survey the existing IIoT testbed landscape. ({\color{red} Raymond: To be continued ...})

\subsection{Questions to be answered}

- A general description of the testbed;

- What type of physical system the testbed is built on;

- What type of wired/wireless technologies are used in the testbed and
what are the key performance metrics?

-  What type of computing facilities are used in the testbed? Gateway,
cloud-based platform? What are the key desired functions and performance
metrics?

- What types of interfaces the testbeds provide to the end users?

-What types security and privacy protection mechanisms are provided in
the testbed?

{\color{red}Raymond: Would be useful to have a couple of summary tables, with different focuses, such as industry sector / application domain (replace the `representative experiments' column in the current Table 1), device types (e.g., drones), estimated device quantity - scale of testbed), types of data / datasets available, open / private testbed, network architecture. An additional column that lists the papers that actually list the respective testbed(s) could also be interesting. }

\section{NIST}

\subsection{NIST IIoT Testbeds}
National Institute of Standards and Technology (NIST), as a national institute, designs and develops many specific concepts to guide the development, operations, and evolution of CPS/IoT testbed to establish cross-sector CPS/IoT testbed. It targets to provide an integrative reconfigurable, reproducible, scalable, and usable across multi-domain CPS and IoT. For example, the Universal CPS Environment for Federation (UCEF) is a software package that enables the creation and management of configurations of the system's experimental components under test~\cite{UCEF}. UCEF is an open-source tool kit that provides a collaborative experiment-development environment~\cite{UCEF1}. 

One of the testbeds from NIST is smart manufacturing systems (SMS)~\cite{helu2020connecting} to support the collection, curation, and re-use of manufacturing data. The testbed is via web-based service with two components: (1) a Volatile Data Stream (VDS) of time-synchronized manufacturing data, and (2) a Queryable Database Repository (QDR) for querying a database containing archived manufacturing data. The primary manufacturing data standard used in the Test Bed is MTConnect. MTConnect is developed by the MTConnect Institute, which is an American National Standards Institute (ANSI)-accredited standards-development organization. MTConnect may be used with a machine-to-machine protocol, such as OPC Unified Architecture (UA). Similarly, MTConnect may be used with pub-sub protocols, such as MQ Telemetry Transport (MQTT). Fig.~\ref{Fig:MTC} provides an overview of the resulting network architecture. Specifically, it includes both wired and wireless connections, and it provides a cloud-based instance. 

\begin{figure*}
  \centering
  \includegraphics[width=15cm]{Figs/MTConnector}
  \caption{Overview of the network diagram that describes the infrastructure deployed in the Test Bed~\cite{helu2020connecting}
  }
  \label{Fig:MTC}
  \vspace{-0.1in}
\end{figure*}

\subsection{NIST Industrial Wireless Systems (IWS) Testbed~\cite{NISTIWST}}
IWS testbed integrates existing and emerging wireless technologies with live physical systems found in factories of all types. The testbed seeks to merge the physical systems and the radio frequency (RF) environment creating a framework for conducting measurements and test methods that advance the effectiveness, reliability, and security of industrial wireless deployments in factories. 
The physical system monitored by sensors connected to wireless communication nodes. Those sensor signals are routed through an RF Environment Model using an RF channel emulator (RFCE).  The IWS testbed RFCE current supports up to eight (8) physical wireless nodes.  The RFCE creates the electromagnetic properties of the factory.  A controller may then act on sensor signals and send control commands to actuators within the factory.  Through this plant-RF-controller interaction, we study the impacts of wireless on the factory operation. The construction of the IWS testbed is currently underway.

\subsection{MSICST: Multiple-Scenario Industrial Control System Testbed~\cite{xu2019msicst}}
This testbed aims to provide a secure testbed for the industrial control system (ICS), which is to discover ICS vulnerabilities and to study and evaluate cybersecurity implementation. It uses a combination of actual physical equipment and software simulations to build the process scenario sand table and use real hardware and software to build the control systems, demilitarized zone, and enterprise zone networks. 

The overall design of MSICTST testbed is based on the Purdue Enterprise Reference Architecture, which includes an enterprise zone, Demilitarized Zone (DMZ), and a control zone. For example, it can be used to rail transit scenarios. In this scenario, it contains PLC to achieve automatic control of the trains and station operations. The PLC communicates with the field equipment through a Modbus RTU, and it is HMI of the entire platform. It is implemented in KingView, which is an integrated system that consists of standard industrial computer software and hardware platforms. 
Another scenario is the smart grid scenario, whose control system is a typical SCADA system. 
For each scenario, the paper provides detailed device information that they used. 

\subsection{Smart Manufacturing Testbed~\cite{candell2020smart}}

\begin{figure*}
  \centering
  \includegraphics[width=15cm]{Figs/SMT}
  \caption{Workcell testbed architecture~\cite{candell2020smart}.
  }
  \label{Fig:SMT}
  \vspace{-0.1in}
\end{figure*}

\begin{figure*}
  \centering
  \includegraphics[width=15cm]{Figs/SMTI}
  \caption{Workcell Testbed Interfaces~\cite{candell2020smart}.
  }
  \label{Fig:SMTI}
  \vspace{-0.1in}
\end{figure*}

This testbed is designed to serve as a platform for the wireless workcell. As shown in Fig.~\ref{Fig:SMT}, it consists of three main subsystems according to their different roles: workcell modules, network components, and measurement devices. It deploys two Universal Robots (UR) UR3 CB-Series robots that serve as actors in the leader-follower use case. The testbed hosts three computers running Ubuntu 18.04 with the robot operating system (ROS) Melodic distribution, where the ROS provides a rich set of options in control functions and peripheral support for UR3.

Each workcell module in the testbed contains one or more built-in Ethernet interfaces. Two Cisco IE-4000 industrial gigabit Ethernet switches serve as the wired network backbone. Ethernet-wireless adapters are used to replace wired connections by enabling wireless communications between modules. Measurement devices collect data including but not limited to manufacturing progress, machine status, link quality, and network health. 
The testbed can implement the precision time protocol (PTP) to provide the sub-microsecond level accuracy across the networked distributed clocks. A Meinberg M900 time server is used as the central PTP master clock that supports the IEEE 1588-2008 (PTPv2) standard.

Fig.~\ref{Fig:SMTI} shows the interfaces between workcell modules. For each interface, a set of protocols is listed for which the use case will be tested. Ethernet is used for baseline performance testing, while wireless local area network (WLAN) protocols such as IEEE 802.11 will be used when a wireless protocol is employed. 

\textit{Also, in its section 3, it provides several past testbeds, e.g., Tennessee Eastman Chemical Factory, Confined Space Gas Sensing Testbed, 3D Gantry System Testbed, Force Seeking Apparatus Testbed, and Dual Robot Machine-Tending Testbed.}

\subsection{ISA100.11a IWN Testbed~\cite{hany2018performance}}

\begin{figure}
  \centering
  \includegraphics[width=9cm]{Figs/ISA100}
  \caption{Testbed Architecture for ISA100.11a IWN~\cite{hany2018performance}.
  }
  \label{Fig:ISA100} 
  \vspace{-0.1in}
\end{figure}

This work presents network measurement of an ISA100.11a industrial wireless network operating in the presence of WiFi interference. The IEEE 802.15.4–based ISA100.11a wireless protocol operates at the 2.4 GHz band for various industrial applications. IEEE 802.11 WiFi also may operate at the 2.4 GHz band for industrial and data applications in the same environment. The existence of IEEE 802.11 wireless network would have a negative impact on the rated performance parameters of the ISA100.11a networks. The testbed contains a radio frequency (RF) channel emulator to replicate the industrial environment. 

Fig.~\ref{Fig:ISA100} shows a testbed architecture, which includes a high-performance programmable logic controller (PLC) to produce an input signal. Its network consists of ISA100.11a wireless sensors and a gateway, and a vector signal generator with an arbitrary waveform output to produce the WiFi interference signal. The system is composed of a single sensor, gateway, and WiFi interferer.

It measures two classes of measurements criteria:
(1) Signal level criteria: root mean square error, average absolute error, normalized peak cross-correlation, and end-to-end delay; (2) Network-level criteria: Packet error rate, average latency, maximum latency, and received signal strength indicator. 

\subsection{Industrial Wireless Sensor Actuator Networks~\cite{brummet2018flexible}}
The network model is based on WirelessHART. Networks consist of a gateway and a set of field devices that include sensors and actuators. Controllers are modeled as being centrally located at the gateway. All nodes are equipped with half-duplex 802.15.4 compatible radios. Consistent with the WirelessHART standard, all nodes are time-synchronized with a slot duration of 10 ms, support 16 communication channels, and respond with an acknowledgment (ack) upon successful packet reception.

They implemented LCP (Link-Centric Policy) and FCP (Flow-Centric Policy) on TelosB motes and evaluated both on a 16 node tested deployed at the University of Iowa. The motes run a TSCH schedule based on plans constructed by the LCP and FCP planners configured with different numbers of retransmissions. 

\subsection{Wireless Factory Workcell~\cite{montgomery2019wireless}}
This document is to provide wireless requirements to realize the benefits of wireless communication systems within factories. It specifies several requirements considerations, e.g., latency, reliability, scalability, range, payload size, update rate, operation and implementation costs, security, and system resiliency. Also, it provides external wireless user requirements, from the perspective of ISA, ETSI, industry. 






\section{IIC Testbeds}

\subsection{LTE for Metro Testbed~\cite{IIC1}}
A metro system is a wireless communication sub-system which carries multiple types of services for train control and management between devices on moving trains and ground facilities. There are four key technology areas found in the rail industry that apply to the LTE for Metro Testbed: QoS, wide-coverage, fast handover algorithm, and anti-interference technology. The LTE for Metro Testbed incorporates the B-Trunking standards of the International Telecommunication Union (ITU), as well as the Urban Rail Train-Ground Integrated Communication System specifications of the China Association of Metros (CAMET).

\subsection{Predictive Maintenance Testbed~\cite{IIC2}}
The testbed’s goal is to develop algorithms and test them in IIoT architectures and real industrial environments. The testbed is with one of Xilinx’s latest technologies. Technologies from iVeia and other vendors of technology make up the testbed’s hardware system.

\subsection{Deep Learning Facility Testbed~\cite{IIC3}}
The IIC Deep Learning Facility Testbed was founded to improve building operational efficiency and occupant satisfaction using AI deep learning techniques, and to share the new-found knowledge within the IIC. 

\subsection{Time-Sensitive Networking Testbed~\cite{IIC4}} 
The IIC’s TSN Testbed endeavors to apply new TSN technology in a manufacturing system with a wide range of automation and control vendors, to display the new capabilities and value of TSN. This deterministic characteristic is important to many industrial automation and control applications for manufacturing in oil and gas, utilities, and transportation. TSN is an enhancement of Ethernet (standards IEEE 802.1 and 802.3 comprise what is generally considered Ethernet) to bring more deterministic capabilities to the network. TSN brings a number of enhancements to Ethernet. TSN comprises a number of enhancements, but three key capabilities form the core of TSN, which includes time synchronization, sending scheduled traffic flows, and central, automated system configuration. 

Besides the above testbeds, the IIC consortium provides many other industrial testbeds, details to refer ``https://www.iiconsortium.org/test-beds.htm"~\cite{IIC0}. 


\section{PAWR Testbeds~\cite{PAWR}}
The Platforms for Advanced Wireless Research (PAWR) program enables experimental exploration of new wireless devices, communication techniques, networks, systems, and services that will revolutionize the nation’s wireless ecosystem while sustaining US leadership and economic competitiveness for decades to come.

\subsection{POWDER-RENEW~\cite{POWDER-RENEW}}
Powder is a remotely accessible ``living laboratory" to enable mobile and wireless research. Powder is deployed in a ``real world" environment/configuration with radio equipment, fiber infrastructure, edge-compute, and datacenter/cloud resources deployed in a ``city-scale" platform.

It provides fixed-endpoint resources. Each Fixed Endpoint (FE) installation in POWDER contains an ensemble of software-defined radio (SDR) equipment from National Instruments (NI) with complementary small form factor compute nodes. There is no wired backhaul, though the platform does provide seamless access via cellular/WiFi to resources in an FE installation. Endpoints are mounted at human height level on the sides of buildings. For example, Antennas is Taoglas GSA.8841 wideband I-bar antenna. Its NI SDR Equipment includes NI USRP B210 SDR on nuc1 and NI USRP B210 SDR on nuc2. 
 

\subsection{COSMOS~\cite{raychaudhuri2020challenge}}
COSMOS - Cloud enhanced Open Software-defined MObile wireless testbed for city-Scale deployment. New wireless communication technologies such as millimeter-wave (mmWave), large/distributed MIMO, and dynamic spectrum access will enable these order-of-magnitude gains and usher in a new era of applications. A major challenge is the lack of a programmable testbed for allowing the academic research community as well as the wireless industry to explore in the most demanding real-world environments the technology sweet sporť of ultra-high bandwidth and ultra-low latency. 
Therefore, there is a need to design a testbed that will enable researchers to conduct accurate experiments over a broad range of new system designs. It should incorporate emerging spectrum techniques (e.g., dynamic spectrum sharing, mmWave, and full-duplex), techniques for Gbps+ radio access such as low latency mobile core network protocols, and edge cloud services. A testbed focusing on high bandwidth and low latency will also provide the capabilities needed for Internet-of-Things (IoT), e-Health, and smart communities applications.

COSMOS is designed to incorporate a fast programmable core network for providing connections across different computing layers. This core network consists of mostly 100 Gbps+ fiber, as well as free-space optical (FSO) and microwave backhaul technologies interconnected with an SDN switching fabric for both minimum latency and flexibility in setting up experimental network topologies. COSMOS integrates advanced optical switching technology based on wavelength- division multiplexing (WDM) switch fabrics and radio over fiber (RoF) interfaces to achieve ultra-low latency connections to edge and central clouds.

The COSMOS SDR nodes in small/medium/large form factors include the same general components (e.g., CPU, FPGA-assisted SDRs, and antennas). To support various experimental capabilities required by the research community, all the radio nodes offer full flexibility of spectrum use in 400 MHz - 6 GHz with a subset of the nodes equipped with 28 GHz mmWave capability.

Another key building block of COSMOS is the IBM 28 GHz phased array antenna module (PAAM), which can enable unique mmWave experimentation at the PHY, link, and network layers with multi-beam support and agile beam steering capability, which is currently not supported by other testbeds. 

A critical building block of COSMOS is the optical transport network and its unique ability to emulate optical front/mid/back- haul (x-haul) networks, which is currently not supported by other testbeds. It is used to enable high bandwidth and low latency networking and to support experimentation with emerging and future wireless technologies and applications.

The edge cloud computing sites contain three types of computing resources: CPUs, GPUs, and FPGAs in order to provide flexible and powerful signal processing capabilities, while also supporting general-purpose computing tasks required for different applications. Software tools are provided to support parallel execution on combinations of CPU/GPU/FPGA. 

The COSMOS control and management software, whose architecture is based on a central controller (similar in concept to SDN), is one of the critical technologies for the successful operation of the testbed.

It also provides an education toolkit at https://www.cosmos-lab.org/cosmos-toolkit/index.php/educational-toolkit/index.html .
In this toolkit, it contains a hardware system and software system. For the hardware system, the hardware setup is a downgraded version of the COSMOS nodes. Consists of various off-the-shelf components that combined together allow the teachers to execute experiments. The hardware setup consists of the following major components: software-defined radio (SDR), processing units, IoT nodes, and the mobile node.
For a software system, it is a web-based interface that has been enhanced with an easy to use philosophy on the execution and management of the experiments since it is designed for K–12 teacher and students. The users are able to select a particular lab, execute the experiment, and collect the measurements with the same operational philosophy as the COSMOS testbed. The software system is divided into the following components: web front-end interface, web back-end server, GNU radio, and IoT management. 

\subsection{PAWR Testbeds – AERPAW~\cite{AERPAW}}
AERPAW, which stands for Aerial Experimentation and Research Platform for Advanced Wireless, was named as the third PAWR testbed in 2019 and is designed with a focus on wireless communications for unmanned aerial systems (UAS) and ground mobility. The AERPAW team is now in the first phase of testbed deployment and expects to make the platform available for early research at the beginning of 2021.

A summary of the broader AERPAW experimentation scenarios is provided in the table~\ref{Fig:AREPAW}.

\begin{figure*}
  \centering
  \includegraphics[width=15cm]{Figs/AREPAW}
  \caption{Experiment setup of COSMOS (preliminary)~\cite{AERPAW}.
  }
  \label{Fig:AREPAW}
  \vspace{-0.1in}
\end{figure*}

\section{Testbeds in Academia}

\subsection{UT San Antonio}

Very little information can be founded online about the testbeds of UT San Antonio. It seems most of these testbeds are from the Institute for Cyber Security (https://ics.utsa.edu/). Or these testbeds (e.g., Building Automation System Testbed) are for internal usage. 



\subsection{WUSTL Wireless Sensor Network Testbed~\cite{WUSTL1}}
Our testbed deployment is based on the TWIST architecture originally developed by the telecommunications group (TKN) at the Technical University of Berlin. The acronym TWIST stands for ``TKN Wireless Indoor Sensor network Testbed". It is hierarchical in nature, consisting of three different levels of deployment: sensor nodes, microservers (i.e., Raspberry PIs), and a desktop-class host/server machine. A high-level view of this three-tiered architecture can be seen in Fig.~\ref{Fig:WUSTLWSNT}.

\begin{figure}
  \centering
  \includegraphics[width=8cm]{Figs/WUSTLWSNT}
  \caption{Testbed Architeture of WUSTL Wireless Sensor Network~\cite{WUSTL1}.
  }
  \label{Fig:WUSTLWSNT}
  \vspace{-0.1in}
\end{figure}

At the lowest tier, sensor nodes are placed throughout the physical environment in order to take sensor readings and/or perform actuation. They are connected to microservers at the second tier through USB cables. Messages can be exchanged between sensor nodes and microservers over this interface in both directions. At the third and final tier exists a switch and a dedicated server which connects to all of the microservers over an Ethernet backbone. The server machine is used to host, among other things, a database containing information about the different sensor nodes and the microservers they are connected to. This database minimally contains information about the connections that have been established between the sensor nodes and microservers, as well as their current locations. The server machine is also used to provide a workable interface between the testbed and any end-users. Users may log onto the server to gain access to the information contained in the testbed database, as well as exchange messages with nodes contained in the testbed. The entire TWIST architecture is based on cheap, off-the-shelf hardware and uses open-source software at every tier of its deployment.

Individual sensor nodes in the testbed can also be disabled or enabled the USB interface. This capability allows node failures to be simulated in the testbed environment, as well as fine-tune the density of the network itself when running certain types of experiments. The introduction of new nodes into the network can also be simulated by enabling nodes at specific times during the run of an experiment.

The testbed software has a client/server architecture, plus a set of user applications that interact with the wireless testbed. The client runs on the microservers and manages finding, programming, and communicating with the attached motes. The server coordinates the clients and user applications. The user applications help the user to program, list, and communicate with motes in the system.

Please keep in mind that the motes deployed in the testbed only contain sensors for light, radiation, temperature, and humidity. There are no microphones or cameras, and there is no plan to EVER include such sensors in the future. The purpose of the testbed is primarily for measuring the communication characteristics of the motes and not evaluating the sensitivity or accuracy of its sensors.

\subsection{WUSTL RT-WCN~\cite{WUSTL2}}
Wireless sensor-actuator networks represent a new generation of communication technology for industrial process monitoring and control. With the adoption of WirelessHART, an open wireless sensor-actuator network standard, recent years have seen the successful real-world deployment of wireless control in process industries. Industrial control systems impose stringent real-time and reliability requirements on wireless control networks. We aim to develop real-time protocols and analysis of wireless sensor-actuator networks (WSANs), particularly those used in control applications. The project goals are three-fold: (1) end-to-end delay analysis for real-time flows sharing a WSAN, (2) network protocols and algorithms for real-time communication over WSANs, and (3) implementation and experimentation of real-time WSANs on a physical wireless testbed. 

The testbed established a novel real-time scheduling framework for wireless control networks based on WirelessHART by bridging real-time scheduling theory and wireless networking.

Wireless sensor-actuator networks (WSANs) offer an appealing communication technology for process automation applications. While industrial WSANs have received attention in the research community, most published results to date focused on the theoretical aspects and were evaluated based on simulations. There is a critical need for experimental research on this important class of WSANs. We developed an experimental testbed by implementing several key network protocols of WirelessHART, an open standard for WSANs widely adopted in the process industries, including Time Slotted Channel Hopping (TSCH) at the MAC layer and reliable graph routing supporting path redundancy. We performed a comparative study of the two alternative routing approaches adopted by WirelessHART, namely source routing and graph routing. Our study shows that graph routing leads to a significant improvement over source routing in terms of worst-case reliability, at the cost of longer latency and higher energy consumption. It is, therefore, important to employ graph routing algorithms specifically designed to optimize latency and energy efficiency. Our studies also suggest that channel hopping can mitigate the burstiness of transmission failures; a larger channel distance can reduce consecutive transmission failures over links sharing a common receiver. 

\subsection{WUSTL REACT~\cite{gunatilaka2020react}}
REACT is a reliable, efficient, and adaptive control plane optimized for adaptation in industrial WSANs. Specifically, REACT integrates two key components.
(a) Reconfiguration Planner employs strategies to compute and update routes and transmission schedules. Designed to minimize the changes to transmission schedules, the planner effectively reduces the latency and energy cost in disseminating a new schedule.
(b) Update Engine provides the mechanisms for network adaptation, including health reporting, failure notification, and an efficient and reliable schedule dissemination mechanism. Our design also allows critical flows impacted by link failures to recover faster than other ones.

The design adopts the IEEE 802.15.4 physical layer, offering a low data rate and low power communication, and operating on the 2.4 GHz band with 16 channels. On top of the physical layer is TSCH MAC protocol. TSCH is a TDMA-based protocol in which time is divided into slots. Each slot is 10 ms, long enough to accommodate the transmission of a packet and its acknowledgment. 

A protocol stack runs on TinyOS 2.1.2 and TelosB motes, and it incorporates features necessary for schedule reconfiguration, including health reporting, failure notification, and TSCH schedule updating into the network protocol stack, which supports TSCH MAC and source routing.

It quantifies the performance of the reconfiguration planner based on two metrics: (1) the success rate in rescheduling a flow without modifying schedules of other flows, and (2) the number of packets required to update flow schedules. For the update engine, we run experiments on the local testbed, present the resulting schedule reconfiguration timelines, and measure the schedule dissemination latency and the energy cost.

\subsection{ISU's NetEye~\cite{ISU1}}
NetEye consists of 130 TelosB motes (with IEEE 802.15.4 radios), 15 Dell Vostro laptops (with IEEE 802.11 b/g radios), and one compute server which are deployed in State Hall --- the Computer Science building at Wayne State University. In addition to providing a local facility for supporting research and educational activities, NetEye is being connected to Kansei as a part of the Kansei consortium; Kansei consortium is initiated to enable experimentation across shared, widely distributed sensor net testbeds at organizations such as Wayne State University, The Ohio State University, Los Alamos National Laboratory, and ETRI, Korea. 

NetEye provides users with a simple, powerful web portal, which streamlines users’ experience in the whole lifecycle of scientific experimentation (e.g., experiment scheduling, status monitoring, and data exfiltration). NetEye employs a stable, fault-tolerant state machine to improve the robustness of the testbed in the presence of failures. NetEye also develops a health monitoring service ``NetEye Doctor” that monitors hardware and software status; the real-time health monitoring information about the testbed is seamlessly integrated with the lifecycle of experiment scheduling, experiment status monitoring, and experiment data analysis for both robust experimentation and for informed experiment analysis. To address the log-data congestion problem in long-running, large scale experiments, NetEye employs a TDMA mechanism to ensure reliability in exfiltrating experiment data to users. To facilitate quick, repetitive scientific experimentation, NetEye also speeds up the mote programming cycle through fast job status transition and multi-thread-based mote programming. NetEye has been successfully running for over 3.5 years, and it has been integrated with federated WSN experimental infrastructure KanseiGenie. 

In NetEye, the laptop is a Dell Vostro 1400 model with an Intel dual-core processor, 1 GB Ram. It is equipped with IEEE802.11a/b/g wireless radio. The operating system on the laptop is the Linux Fedora that runs on a 24/7 basis. The 15 laptops are physically arranged on 15 wooden benches which are customized for NetEye deployment and spaced from each other properly.

The sensing element — TelosB mote in NetEye, is an open-source platform designed to enable the application deployment for experimentation. It is an IEEE802.15.4 compliant device designed by UC Berkeley and manufactured by Crossbow Solutions. Each TelosB mote is equipped with a T1 MSP430 microcontroller, a 2.4 GHz Chipcon CC2420 radio, 4MHz 8bit CPU, 48KB instruction memory, 10KB RAM, and a USB interface. The radio’s reliable transmission range is roughly between 20m to 30m when placed in an indoor environment. Each mote accommodates a light sensor. The motes run TinyOS 2.1 that is a light-weight and event driven operating system which implements the networking stack and communication with sensors, and provides the programming environment for the platform.

The related works section provides lots of useful information (NetEye- A User-Centered Wireless Sensor Network Testbed for High-Fidelity, Robust Experimentation).


\subsection{ISU's Kansei~\cite{ISU2}}

Consisting of 210 Extreme-Scale Motes (XSM) and 210 Extreme Scale Stargates (XSS), Kansei provides a testbed infrastructure to conduct experiments with both IEEE 802.11 and 802.15.4 mote networks. The testbed is composed of 210 Extreme-Scale Motes (XSM) and 210 Extreme Scale Stargates (XSS). The design of the 210-node 802.11 network is such that link and network properties in Kansei mimic those outdoors.

The testbed features an experiment scheduler designed for flexible and dependable experimentation. The hardware and software platforms for Kansei have been set up to facilitate high-fidelity wireless network experimentation. This includes studying both indoor and outdoor wireless link properties and co-designing the network system to enable high-fidelity experimentation with reconfigurable network setup, such as node distribution density and wireless link reliability.

The hardware infrastructure of Kansei consists of three components: Stationary Array, Portable Array, and Mobile Array. (1) The stationary array consists of 210
sensor nodes placed on a 15×14 rectangular grid benchwork
with 3ft spacing. Each node in the stationary array consists
of two hardware platforms: Extreme Scale Motes (XSMs)
and Stargates.  

\subsection{WSU's NetEye~\cite{WSU}}
It seems this testbed is the same as ISU's NetEye, which is a collaborative project. 

\subsection{WSU's SNOW~\cite{SNOW}} 
SNOW is Sensor Network Over White Spaces. It seems this is for TV white space (where TV transmissions are in lower frequencies – VHF and lower UHF (470 to 698MHz)), which is not a real testbed for industrial cases. 
SNOW is the design of a highly scalable low power and long-range wireless sensor network over the TV white spaces. At the heart of its design is a Distributed implementation of Orthogonal Frequency Division Multiplexing (OFDM), called D-OFDM. The base station splits the wide white space spectrum into narrowband orthogonal subcarriers allowing D-OFDM to carry parallel data streams to/from the distributed nodes from/to the base station. Each sensor uses only one narrow-band radio. The base station uses two wide-band radios, one for transmission and the other for the reception, allowing transmission and reception in parallel. Each radio of the base station and a sensor is half-duplex and equipped with a single antenna. SNOW supports reliable, concurrent, and asynchronous receptions with one single-antenna radio and multiple concurrent data transmissions with the other single-antenna radio. This is achieved through a new physical layer design by adopting D-OFDM for multiple access in both directions and through a lightweight MAC protocol. While OFDM has been embraced for multiple access in various wireless broadband and cellular technologies recently, its adoption in low power, low data rate, narrowband, and sensor network design is novel. Taking advantage of low data rates and short payloads, we adopt OFDM in SNOW through a much simpler and more energy-efficient design.

In SNOW, a subcarrier bandwidth can be chosen as low as 100kHz, 200kHz, 400kHz depending on the packet size and expected bit rate. Using a subcarrier, a sensor node can have several kilometers of transmission range at 0dBm. Using a single base station, SNOW has the capability of supporting millions of devices. As an added advantage, it can use a fragmented spectrum of white spaces. We implemented SNOW on two hardware platforms -- USRP using GNU radio and TI CC1310. CC1310 is a tiny, cheap (<\$30), and commercially off-the-shelf (COTS) device with a programmable PHY. We implemented SNOW with CC1310 (using CC-ANTENNA-DK2 antenna) as a node, and the BS is a USRP210 with a laptop.

Currently, we have a temporary SNOW testbed of 43 nodes for experimental purposes that co-locate with our permanent wireless sensor network (WSN) testbed at Wayne State University. Specifically, we have 43 SNOW nodes of which 34 are based on CC1310 and 9 are based on USRP which are co-located with our WSN testbed.

\subsection{Binghamton's Testbed~\cite{BUT}}
There are no more new testbeds, which is mainly based on the testbed provides by WUSTL's WSAN for industrial. 

\subsection{Northeastern's Colosseum~\cite{Colosseum}}
Colosseum is the world’s largest radio frequency channel emulator, designed to support research and development of large-scale, next-generation radio network technologies in a repeatable and highly configurable RF environment. It combines 128 Standard Radio Nodes (SRNs) with a Massive digital Channel Emulator (MCHEM) backed by an extensive FPGA routing fabric. Each of the SRNs provides a platform for Software Defined Radio as well as Machine Learning applications with two key hardware components, namely, a Dell R730 Server which comes with an NVIDIA K40M GPU, and an Ettus Research USRP X310 Software-defined Radio that is equipped with a XILINX Kintex 7 FPGA. The MCHEM facilitates real-world wireless RF channel emulation between the SRNs and can emulate fading, multipath, etc., for up to 256 x 256 independently customizable channels. This allows for large scale RF testing with up to 256 independent radio nodes, each with powerful computational capabilities. Accessible as a cloud-based platform, Colosseum also provides other resources to create a real-time high-fidelity radio scenario such as traffic generation, timing, and GPS synthesis.

Colosseum is a massive RF and computational facility that emulates wireless signals (with granularity at the RF signal level) traversing space and reflecting off multiple objects and obstacles as they travel from transmitters to receivers. Allowing 256 x 256 100 MHz RF channel emulations, with USRP X310 radio nodes in the loop interacting in over 65,000+ channels at the same time, Colosseum can create virtual worlds, as if the radios are operating in an open field, urban area, shopping mall, or a desert, by generating more than 52 terabytes of data per second. Colosseum enables full-stack wireless networking research from applications down to the physical layer at scale - with up to 256 interacting radios.

As an RF testbed Colosseum can be utilized to:

$\bullet$ Emulate multiple operational environments including a 1 sq. km open field, a dense urban city, a suburban shopping mall, a desert, or anything in-between. 
$\bullet$ Emulate in real-time multipath and fading effects with high-fidelity ray-tracing.
$\bullet$ Support high-fidelity and large-scale research on waveforms, protocols at all layers, networked applications, jamming and security, MIMO, and beamforming.
$\bullet$ Provide full-stack repeatable environment (from RF to application layer).
$\bullet$ Carry out large scale testing, up to 256 radio nodes with 256x256 configurable channels.
$\bullet$ Support cellular networks (4G, 5G), IoT, cognitive radio, ad hoc networks, edge computing, and cloud RAN research.
$\bullet$ Implement Machine Learning algorithms in different wireless communications techniques such as spectrum sharing, dynamic spectrum access, extraction of signal intelligence and optimized routing, by providing built-in powerful computational resources.
 

Colosseum provides users with preconfigured and ready to use LXC containers for basic testing. Users can customize these containers based on their needs to develop and implement their own radio codes. These customized container images can be uploaded to the Colosseum servers, and the user may choose to load the default or the customized containers onto the SRN's during their reserved session. This allows for completely customizable RF testing with a variety of repeatable scenarios that enables the users to conduct virtually any type of research on waveforms and different layers of protocol stack as well as networked applications, among others.



==> sec/tsn/tsn_other.tex <==
\subsection{Legacy Network Testbeds}

This section transitions from the discussion of TSN to an examination of traditional industrial Ethernet protocols such as PROFIBUS, EtherCAT, and TTEthernet. These legacy networks, while not incorporating TSN capabilities, have been foundational in the development of industrial Ethernet and merit thorough exploration.

\input{Tables/tsn/others}

\subsubsection{PROFINET}
%\hfill\\

\textbf{Flammini et al.} \cite{ferrari2011large} constructed a PROFINET IO RT network to enhance simulation models and validated critical scenarios in real-world testbeds. PROFINET IO RT, designed for unsynchronized, best-effort communication, has performance contingent on the network design and operating conditions. The network features a ring backbone with 11 switches, 115 IO-Devices, and a single IO-Controller, directly attached to the ring switches or connected to drops, with a maximum drop length of nine devices as shown in Fig.~\ref{Fig:TSN:profinent}. Configuring the switches as IO-Devices results in a total of 127 PROFINET IO-enabled devices. Despite operating under heavy load, the devices maintain commendable timeliness, with the standard deviation of the data exchange period from IO-Device to IO-Controller under 50 microseconds.
\eat{
\begin{figure}
  \centering \includegraphics[width=\linewidth]{Figs/lagacy/profinent.png}
  \caption{The PROFINET IO RT real-world testbeds.}
  \label{Fig:TSN:profinent}
\end{figure}
}

\subsubsection{EtherCAT}

%\hfill\\

\textbf{Delgado et al.} Delgado et al. constructed an EtherCAT-based servo motor testbed to examine the minimum cycle time for microgrid applications \cite{delgado2018application}. The testbed consists of a master, powered by an Intel Atom D2700 CPU and Realtek RTL8169 Gigabit NIC, and six servo motors acting as slaves, connected via CANopen-over-EtherCAT as shown in Fig.~\ref{Fig:TSN:grid}. Each motor is configured to transmit 24 Bytes of process data objects per iteration. The experiments revealed a minimum cycle time of 322.269 microseconds in a 100 Mbps setup, accounting for the worst-case execution time.

\begin{figure}
  \centering \includegraphics[width=\linewidth]{Figs/lagacy/microgrid.png}
  \caption{An EtherCAT-based servo motor testbed with six servo motors acting as slaves.}
  \label{Fig:TSN:grid}
\end{figure}

\textbf{FastCat.} \cite{brinkman2021fastcat} developed Fastcat, an open-source C++ library for EtherCAT device configuration, designed for testbed and robotic applications. Fastcat offers various features, including support for multiple EtherCAT Masters, a YAML input configuration file, and a visualization tool called 'Fcviz' for bus topology mapping using the Graphviz library. It facilitates efficient data routing and command control between devices, enabling self-contained closed-loop systems like heaters or joint-torque controllers without added latency. Fastcat has been implemented in two applications in NASA Jet Propulsion Laboratory (JPL): a gripper control testbed and a sampling chamber testbed. The paper, however, does not specify the number of nodes used in these testbeds.

\begin{figure}[ht]
    \centering
    \begin{minipage}[b]{0.23\textwidth}
    \includegraphics[width=\textwidth]{Figs/lagacy/gripper.png}
        \caption{JPL gripper control testbed.}
        \label{Fig:TSN:gripper}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.23\textwidth}
    \includegraphics[width=\textwidth]{Figs/lagacy/chamber.png}
        \caption{JPL chamber testbed.}
        \label{Fig:TSN:chamber}
    \end{minipage}
\end{figure}

\textbf{Edelberg et al.}
JPL developed the Sampling and Caching Subsystem (SCS) development testbeds for the Mars 2020 Rover Mission, serving as a hardware and software integration prototype for testing~\cite{edelberg2018software}. EtherCAT was chosen as the communication bus for its low jitter and high bandwidth. The SCS testbed tests a subset of components, including a robotic arm, coring drill, adaptive catching assembly, and gas dust removal tool. Beckhoff EtherCAT modules are used for all nonactuator I/O, including reading force-torque sensor strain gauges, toggling digital outputs, etc. 

\eat{
\begin{figure}
  \centering \includegraphics[width=\linewidth]{Figs/lagacy/scs.png}
  \caption{SCS}
  \label{Fig:TSN:scs}
\end{figure}
}
\subsubsection{TTEthernet}



\textbf{Yu et al.}
In \cite{yu2017handling}, a novel traffic shaping approach is proposed to address scheduling uncertainties in TTEthernet and implemented on an actual TTEthernet testbed. This approach buffers early frames and releases them at their pre-scheduled arrival times during fault scenarios. The testbed comprises three time-triggered switches in a linear topology and two IXIA 400T traffic generators, creating a time-triggered train network. The switches provide fault tolerance with 24 ports, implemented using FPGA, while IXIA 400T generates specific real-time frames with fixed periods, ensuring clock precision within 10 nanoseconds. The network's total bandwidth is 100Mbps, and devices achieve clock synchronization precision of 200 $ns$ using IEEE 1518.

\eat{
\begin{figure}
  \centering \includegraphics[width=\linewidth]{Figs/lagacy/shaper.png}
  \caption{Shaper}
  \label{Fig:TSN:shaper}
\end{figure}
}

%\hfill\\

\textbf{Loveless et al.} 
In \cite{loveless2015ttethernet}, the application of TTEthernet technology to future spacecraft is explored through the development of two integrated testbeds demonstrating network failover via redundancy links. This research aims to guide the implementation of onboard communication systems on the NASA Orion vehicle. The TTEthernet-based flight control loop, located in Bay 1 of the IPAS testbed, features two redundant failover-capable flight computers, a corresponding Trick simulation machine, and two parallel switches offering redundant paths as seen in Fig.\ref{Fig:TSN:arm}. The other testbed illustrates the TTEthernet failover architecture used in the AA2 flight test during the A\&S project’s May FY15 Integrated Test, shown in Fig.\ref{Fig:TSN:aa2}, where redundant switches bolster network fault-tolerance.

\begin{figure}[ht]
    \centering
    \begin{minipage}[b]{0.23\textwidth}
    \includegraphics[width=\textwidth]{Figs/lagacy/ARM.png}
        \caption{IPAS testbed}
        \label{Fig:TSN:arm}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.23\textwidth}
    \includegraphics[width=\textwidth]{Figs/lagacy/AA2.png}
        \caption{AA2 flight test}
        \label{Fig:TSN:aa2}
    \end{minipage}
\end{figure}




% \begin{itemize}
%     \item Fieldbus-based: Modbus, PROFIBUS, CAN. (optional)
%     \item Ethernet-based: Modbus/TCP, PROFINET, EtherCAT, Powerlink, TTEthernet, TSN. (\textbf{Chuanyu})
% \end{itemize}

